Floorplet: Performance-aware Floorplan Framework for Chiplet Integration

A chiplet is an integrated circuit that encompasses a well-defined subset of an overall system's functionality. In contrast to traditional monolithic system-on-chips (SoCs), chiplet-based architecture can reduce costs and increase reusability, representing a promising avenue for continuing Moore's Law. Despite the advantages of multi-chiplet architectures, floorplan design in a chiplet-based architecture has received limited attention. Conflicts between cost and performance necessitate a trade-off in chiplet floorplan design since additional latency introduced by advanced packaging can decrease performance. Consequently, balancing power, performance, cost, area, and reliability is of paramount importance. To address this challenge, we propose Floorplet, a framework comprising simulation tools for performance reporting and comprehensive models for cost and reliability optimization. Our framework employs the open-source Gem5 simulator to establish the relationship between performance and floorplan for the first time, guiding the floorplan optimization of multi-chiplet architecture. The experimental results show that our framework decreases inter-chiplet communication costs by 24.81%.

==> doc/answer.tex <==
{
\onecolumn
%\normalsize

\noindent\textbf{Responses to reviewers and editor}

\section*{\textbf{Reviewer 1}}

\begin{commentblock}{Summary}
The authors proposed a Chiplet floorplanning algorithm considering performance and reliability issues. With three steps optimizations, the chiplet floorplan generated by the proposed method can outperform SOTA work in terms of performance and power. The work is solid and important for Chiplet design. Some questions and concerns are listed as follows,
    
\end{commentblock}
\textbf{Response:} 
Thanks for your constructive feedback. 
We highly appreciate your recognition of the importance of the research topic and your positive evaluation of our work.
we have carefully polished the manuscript and added more experiments according to your suggestions. 
The detailed solutions for specific questions are listed below.


\begin{commentblock}{1-1}
The author obviously omitted one important literature ``GIA: A Reusable General Interposer Architecture for Agile Chiplet Integration" (ICCAD 2022). This work also discussed floorplanning optimizations of Chiplet. They even talked about the reusage of the interposer and thermal problems, which are important but unfortunately not mentioned or considered in your work. The authors should compare the work with this relevant work.
\end{commentblock}
\textbf{Response:}
We sincerely appreciate the valuable comments. 
We provide a more comprehensive literature review of previous work \cite{Chiplet-GIA-ICCAD2022-Li} in this version.
Through comparing with the work, we elaborate on the motivation of Floorplet and emphasize the insights of our work.

\begin{itemize}
    \item The differences between the GIA and the Floorplet.
Work~\cite{Chiplet-GIA-ICCAD2022-Li} utilizes the modular design on the interposer, which means that each chiplet is placed on the tiles with an equal size on the interposer. 
This scheme improves the re-usability of each chiplet IP, while it may increase the potential of extensive interposer area cost due to unused tiles on the interposer.
In our framework, we adopt a distinct approach for chiplet floorplanning.
The floorplan scheme in our work does not involve routers in the interposer. 
Instead, we attempt to add more flexibility to the routing wire in the interposer and minimize the interposer area to reduce cost.
This approach is motivated by the high cost of the interposer resulting from its large area and correspondingly high defect density. 
Our framework can leverage the router-free approach to widen the floorplan solution space and obtain optimal floorplan solutions for chiplet-based architectures.
    \item The thermal issue is discussed in the Comment 1-2.
    
\end{itemize}

\textbf{Action:} To provide a comprehensive background of the chiplet floorplan in our work, we add more description and compare it with GIA \cite{Chiplet-GIA-ICCAD2022-Li}  in  \Cref{sec:prelim-floorplan}, Paragraph 2, Line 1. 


\begin{commentblock}{1-2}
    Thermal problem is an important consideration for 2.5D and 3D IC design. The authors should consider or at least discuss how the thermal issue is considered in your framework.
\end{commentblock}
\textbf{Response:}
Thank you for the suggestion of considering the thermal issue.

The thermal issue is important in 3D IC or chiplet-based 2.5D IC.
The main reason is the thermal can not be dissipated well with materials in the vertical direction.
Some works have built the thermal model in their work to simulate the heat flow in 3D IC.
An accurate thermal model is constructed based on the actual physical parameters of the packaging.
Our method focuses on introducing performance metrics into the floorplan stage to obtain an early optimization result, so the information related to thermal (\textit{e.g.}, voltage, accurate power) is not available in the current situation platform.

For future work, we plan to extend our framework with some thermal modeling tools like that used in\cite{Chiplet-GIA-ICCAD2022-Li}.
Firstly, we will utilize a thermal simulation model to set the threshold, and after the first stage optimization, the \textbf{optChiplet} will continue to optimize the floorplan.
Even if our current framework doesn't take into account the thermal effect, we hope the idea of combining reliability, technology, and performance can bring more architecture insights into the IC manufacturing community.

\textbf{Action:}
We have added more discussion about thermal issues in our framework in the newly added \Cref{sec:discus-thermal}.

\begin{commentblock}{1-3}
    How interposer delay is modeled is not very clearly presented in your work. As far as I know, the interconnect on the interposer has a strong inductive effect and cannot use RC RC-based interconnect model for delay calculation. What is your delay model and how you verify the correctness of your model is not mentioned in your work.
\end{commentblock}
\textbf{Response:}
Thanks for your suggestion of adding more description of the delay model.


In our framework, we take the conclusion from the work \cite{kim2020chiplet-64core-riscv} to model interposer delay. 
The work designed and constructed a chiplet-based 64-core processor to illustrate the chiplet design flow.
In the Sec. V-B ``Interposer Timing and Power Analysis" of the work, the author evaluates their delay model consisting of resistance, inductance, conductance, and capacitance (RICC). 
According to the results in this work, in the 0.2 to 10.0mm length range, as the wire becomes longer, both communication delay and energy increase linearly. 
In our experiment, the wire length falls into the wire length range mentioned above.
Since the work has verified their conclusion, we consider using this conclusion to build our interposer delay model.
It is difficult to input all parameters (\textit{i.g.}, RICC) from complex circuits into our simulation model, so we utilize the conclusion from \cite{kim2020chiplet-64core-riscv}.


\textbf{Action:}
We have added more information about the delay model in \Cref{sec:method-simChiplet}, paragraph 4, Line 1.

\begin{commentblock}{1-4}
   The floorplanning algorithm is not compared with some existing floorplan algorithms either e.g., B*Tree, SP, CBL, etc. What is your algorithm's timing complexity and how scalability of your algorithm compared with the above methods?

\end{commentblock}
\textbf{Response:}
Thanks for the suggestions for clarifying the differences between our method and some traditional algorithms and analyzing time complexity. 

\begin{itemize}
    \item The differences between our framework and the traditional algorithms.
The main differences between our framework and the algorithms like B*Tree, SP, CBL,\textit{etc} lay in the complexity of the problem constraints.
The constraint of the bump stress is expressed in \Cref{equ: bump constraints} and shown in the left lower corner of \Cref{fig:chiplet-simulation}. 
Most floorplan works like \cite{liu2014chiplet-floorplan,osmolovskyi2018chiplet-placement} do not consider reliability issues in the 2.5D package, \textit{i.e.}, considering the warpage threshold and avoiding the overlap between chiplets and the hotspot bumps.
After introducing reliability in our framework, methods like the enumeration-based algorithm \cite{liu2014chiplet-floorplan}, the branch-and-bound algorithms~\cite{osmolovskyi2018chiplet-placement}, and the other traditional algorithms like B*Tree, SP, and CBL cannot fulfill the problem property.
    \item The motivation of mathematical programming (MP) methods.
Adopting the mathematical programming (MP) methods in our framework can solve problems with multiple complex constraints well.
The MP methods can take complex constraints like warpage threshold, bump reliability, interposer area, and the wirelength into consideration simultaneously during the iterative optimization.
Meanwhile, the solutions to the MP problems can be finished by some excellent solvers like Gurobi\cite{2018gurobi}.
Therefore, we choose to compare our methods with MP-based methods in \cite{zhuang2022multi-package}, and the result illustrates that our methods outperform previous work and achieve a better performance-aware floorplan solution.

    \item Time complexity of the method.
The timing complexity can not be analyzed precisely in the MP-solver-based optimization framework.
That is because the optimization problems in our framework are solved by existing the MP solver Gurobi, so the timing complexity is highly reliant on the solver.
However, we can obtain the running time of the solver for different tasks.
For simple chiplet-based architecture like $\mathcal{C}_{8},\mathcal{C}_{16}$, the whole optimization process can be finished in 20 minutes to 1 hour. 
However, for larger architecture like $\mathcal{C}_{22},\mathcal{C}_{30}$, to obtain a relative optimal solution will take 8-10 hours.

    \item The scalability of our methods.
Our methods have good scalability to handle different chiplet-based architectures with various numbers of chiplets. 
For some common chiplet-based architecture with 10 $\sim$ 30 chiplets, our framework can give a good solution in an acceptable time compared to some traditional methods like the simulated annealing algorithm.
    
\end{itemize}

\textbf{Action:} We have added more discussion on the mathematical programming methods with some traditional floorplan algorithms in the newly added \Cref{sec:discus-tradition}.



\begin{commentblock}{1-5}
    The architecture information is also not clearly presented, such as whether NoC is used in your gem5 simulation. How do you derive the communication latency, based on the task graph or your assumptions?
\end{commentblock}
\textbf{Response:}
We sincerely appreciate the valuable comments.

\begin{itemize}
    \item NoC Simulation. 
In the original simulation tool, network-on-chip (NoC) in Gem5 garnet3.0 combines different modules in the chiplet-based architecture.
The NoC module in gem5 is used to record the data request and data volume, which can assist in obtaining the data movement between chiplets.
However, the original framework does not support setting various latencies between different chiplet-pair flexibly, so we improve the flexibility of the original topology by embedding the latency weight given by the latency-wirelength model in \Cref{fig:latecny-wire-b}. 
    \item Communication latency.
Communication latency between different chiplet-pair is obtained based on the wire-latency model~\cite{kim2019chiplet} in \Cref{fig:latecny-wire-b} according to the spatial location in RDLs.
Currently, the graph is not introduced to our framework, but it can be a promising direction to represent the location of chiplets.
In our extension work, we will consider introducing more chiplet representation methods (\textit{e.g.}, graph) in our framework.

    
\end{itemize}




\textbf{Action:} We have updated the manuscript by adding more details about the architecture simulation in \Cref{sec:method-simChiplet}, Paragraph 1, Line 7.

\begin{commentblock}{1-6}
    Some typos are listed and the authors need to check the manuscript more carefully, e.g., line 17 page 2, 2.5 package should be ``2.5D package", line 14 on page 1 oIC should be ``IC".
\end{commentblock}
\textbf{Response:}
Thanks for your careful checks.
We have thoroughly checked the grammar and fixed all grammar issues in this revision.   

\section*{\textbf{Reviewer 2}}

\begin{commentblock}{Summary}
This work proposes Floorplet, a performance-aware framework for co-optimizing the floorplan and performance of chiplet-based architecture, which aims to address the challenges and drawbacks of using chiplets for complex circuit systems.
The authors developed parChiplet to partition realistic SoC into functional chiplets, a simulation platform simChiplet to evaluate the performance impact of different floorplan solutions and a floorplan framework optChiplet for chiplet-based architecture to consider reliability, cost, area, and power metrics.
The experimental results show that the framework outperforms previous methods.
\end{commentblock}

\textbf{Response:}
Thanks for your constructive feedback to help to improve this work. 
We have carefully polished the manuscript and added more experiments according to your suggestions. 
The detailed solutions for specific questions are listed below.

\begin{commentblock}{2-1}
In Sec. III-B, the algorithm to partition chiplets from the SoC lacks a more detailed description. For example, what are the inputs to the methodology, can it be implemented automatically, and can it be generalized sufficiently across different SoC designs?
\end{commentblock}
\textbf{Response:}
Thanks for your suggestions of adding more detailed descriptions of the algorithm. 


The algorithm is straightforward to process the SoC hierarchical tree recurrently.
The input of the algorithm is the synthesis results given by Hammer~\cite{liew2022hammer} from different SoC designs. 
For various SoC designs, once given the synthesis results, the hierarchical tree can be constructed automatically with function integrity and area information.
Since we have designed the parser to analyze the chiplet interconnection relationship, the algorithm can be generalized across different SoC. 

\textbf{Action:} The descriptions are added in \Cref{sec:method-parChiplet}, Paragraph 5, Line 2.


\begin{commentblock}{2-2}
In Sec.~III-B, what is the purpose of the chiplet pool? The authors mentioned in Sec. IV. that each SoC is divided into 10 $\sim$ 50 chiplets and forms a chiplet pool consisting of about 300 chiplets, but a more specific description is still lacking.
\end{commentblock}

\textbf{Response:}
Thank you very much for the valuable comment. 

The chiplet pool is constructed with various SoCs to avoid time-consuming synthesis design. 
Once we meet the same chiplet components, \textit{i.e.,} IPs, in the new chiplet-based architecture, we can reuse the physical information.
Building a chiplet pool provides an opportunity to reuse the synthesis results from Hammer to avoid the extra process of synthesizing.


\textbf{Action:} 
We have added a more specific description of the chiplet pool in \Cref{sec:exp-benchmark}, Paragraph 2, Line 3.
Furthermore, we constructed a table to show the specific chiplet in \Cref{tab:chiplets}.

\begin{commentblock}{2-3}
In Sec. III-D, the definitions of $ p_{i, j} $ and $ q_{i, j} $ are not clear enough. How do they indicate the relative position between the two Chiplets?
\end{commentblock}

\textbf{Response:}
Thanks for the recommendations for clarifying the denotations. 

In this part, $p_{i,j}$ and $q_{i,j}$ in \Cref{equ: no-overlap-1} $\sim$ \Cref{equ: no-overlap-2} are a pair of indicators with four possible values, which can be adjusted during the \textbf{optChiplet}, \textit{i.e.} floorplan process to add constraints of the relative location of chiplet. 
For example, 
if $(p_{i,j},q_{i,j})=(0,0)$, the chiplet $c_{i}$ is constrained to place on the left of chiplet $c_{j}$; 
if $(p_{i,j},q_{i,j})=(0,1)$, the chiplet $c_{i}$ is constrained to place on the bottom of chiplet $c_{j}$; 
if $(p_{i,j},q_{i,j})=(1,0)$, the chiplet $c_{i}$ is constrained to place on the bottom of chiplet $c_{j}$; 
if $(p_{i,j},q_{i,j})=(1,1)$, the chiplet $c_{i}$ is constrained to place on the top of chiplet $c_{j}$.
In other words, by optimizing this pair, we can change the location of various chiplet to avoid overlap between chiplets.


\textbf{Action:} We add more description following \Cref{equ: no-overlap-2}, \Cref{sec:method-optChiplet}, Paragraph 3.

\begin{commentblock}{2-4}
In Sec. III-D, Equation (18) does not correspond exactly to the description, i.e., area ($ a_{ck} $) vs.  … + $ \beta_2 \alpha_p $ + …. I think the authors should double-check and correct all equations and symbols.

\end{commentblock}

\textbf{Response:}
Thank you for pointing out the inconsistent part of the equations. 


\textbf{Action:} We have thoroughly checked the denotations in the paper and corrected the part that may be ambiguous. 
We also add a table of the notations used in our \textbf{optChiplet} are listed in \Cref{tab:notations} in this version.

\begin{commentblock}{2-6}
In addition, there are some typos in the manuscript that need to be revised:

- In Sec. I, “… to reduce oIC costs …” $\rightarrow$ “oIC” is a typo?

- In Sec. I, “We tested our framework on various benchmarks and show that …” $\rightarrow$ “showed”?

- All acronyms should be given an expansion the first time they appear, e.g., D2D.

- In Sec. III.C, “… elaborated it in III” $\rightarrow$ “… Sec. III”.
\end{commentblock}

\textbf{Response:}
We sincerely thank the reviewer for careful reading.
We correct all the typos in the paper and utilize some grammar tools to assist in solving word issues.   

\section*{\textbf{Reviewer 3}}

\begin{commentblock}{Summary}
This paper proposes a framework for co-optimizing floorplan and performance for chiplet-based designs. The framework consists of 3 parts: an algorithm for partitioning monolithic SoC into chiplets with specific functions, a simulation platform based on Gem5 that evaluates the performance of different floorplan solutions for chiplet-based architecture and a floorplan framework for chiplet architecture that considers performance in addition to reliability, HPWL and package area. The key novelty of this paper is that it considers realistic chiplets with complex data flow and incorporate performance into floorplan optimization. The optimization of performance is achieved by considering communication patterns of workloads during floorplan process to mitigate communication cost and thus reduce clock cycles for finishing a workload. The proposed framework outperforms a previous approach in terms of HPWL, communication cost and latency on 4 SoC architectures while running different workloads.
\end{commentblock}

\textbf{Response:}
Thanks for your constructive feedback to help to improve this work. 
We have carefully polished the manuscript and added more experiments according to your suggestions. 
The detailed solutions for specific questions are listed below.

\begin{commentblock}{3-1}
The idea of the proposed framework is to reduce the latency of finishing a workload by optimizing the floorplan solution of a chiplet-based SoC based on the communication pattern between chiplets when running that specific workload. Such an idea seems to be unreasonable for chiplet-based CPUs (as mentioned in Section IV, part A, paragraph 2) because a CPU can run many different workloads. If the floorplan of a chiplet-based CPU is optimized for one specific workload, it may cause performance degradation when running another workload with a very different communication pattern.  


\end{commentblock}

\textbf{Response:}
Thank you for the comments on the optimization of SoC and the corresponding workloads.

\begin{itemize}
    \item The application-specific SoC.
To boost the computation capability of the SoC architecture, different SoCs are designed specifically with the target of optimizing different applications. 
For instance, \cite{SoC-ISCA2021-Jang} specifically designs the architecture for optimizing DNN applications on flagship mobile devices. 
\cite{SoC-JSSC2011-Sridhara} designs an SoC architecture for mapping medical applications.
Therefore, to optimize the performance of these function-specific chiplet-based architectures, we design the corresponding workloads to do evaluations.
    \item The workloads for specific SoC.
For chiplet-based DNN accelerators, we utilize ResNet-15\cite{he2016resnet}, and MobileNet-v2\cite{howard2017mobilenets} as the workloads. We also use the parallel matrix multiplication workloads, which are the basic operations of DNN-targeting SoC. 
For chiplet-based general-purpose processors, we utilize some representative workloads from the commonly used CPU benchmark SPEC2006\cite{henning2006spec}.
The benchmarks encompass a diverse set of applications with varying performance characteristics, effectively covering the stats of all chiplets.
The workloads for various chiplet-based architectures are listed in \Cref{tab:workloads}. 
    \item The evaluation method of performance.
The chosen workloads are utilized to show the effect of the proposed framework. 
We have run many workloads to obtain the average latency for the architecture.
The data movement frequency between chiplets is the average of various benchmarks that are suitable for the specific SoC design. 
The reported latency is also the average latency of the chosen workloads for many time.
Therefore, the workloads can reflect the performance of the chiplet-based architecture to a large degree.
    
\end{itemize}





\textbf{Action:} 
We have added more description of the SoC and the workloads in \Cref{sec:exp-benchmark}, Paragraph 4 $\sim$ 5.

\begin{commentblock}{3-2}
4 SoC architectures are used in the experiments but the authors don’t give detailed information about the SoC architectures or the functions of the obtained chiplets.

\end{commentblock}

\textbf{Response:}
We sincerely thank the reviewer for the reminder. 
The $\mathcal{C}_{8},\mathcal{C}_{16},\mathcal{C}_{22},\mathcal{C}_{30}$ are partitioned from a SmallRocket core with the corresponding caches and peripheral modules, a MediumBOOM core with the corresponding caches and peripheral modules, a LargeBOOM core with peripheral modules, and a Gemmini accelerator with the processor core, caches and corresponding DMA controllers.

\textbf{Action:} 
We give more information on different SoC designs in \Cref{sec:exp-benchmark} Paragraph 1, Line 5.
Moreover, we provide more data on the obtained chiplets in \Cref{tab:chiplets} with function. 

\begin{commentblock}{3-3}
The authors only provide vague information about the benchmarks used in the experiments. For example, ‘For the CPU architecture, we select some representative workloads from the commonly used CPU benchmark SPEC2006’ (Section IV, part A, paragraph 2).
\end{commentblock}

\textbf{Response:}
We sincerely thank the reviewer for the reminder. 
The benchmarks are from the RISC-V benchmark, SPEC2006 benchmark, and DNN workloads orderly.

\textbf{Action:} We have added detailed information in \Cref{sec:exp-benchmark}, Paragraph 5 for the benchmark used in our experiments.
We also provide a table of benchmarks in \Cref{tab:workloads}.



\begin{commentblock}{3-4}
The area of each chiplet is determined in the SoC partition process. Varying the width and height of a chiplet while keeping the area unchanged would affect the floorplan solution. It could be better if the authors could explain how the original width and height of each chiplet are determined.
\end{commentblock}
\textbf{Response:}
Thank you for the reminder. 
For practical chiplet fabrication, it is very time-consuming to decide on the specific design for each chiplet. 
Only after we obtain the final design of the chiplet, the width, and height can be fixed.
For our experiment, we can not carefully design each chiplet one by one.
Therefore, we simplified the process by generating chiplets with a random width/height ratio within a rational range.
Our framework is capable of handling practical chiplet whatever the width/height ratio.

\textbf{Action:} 
We have provided more information on the width and height from \Cref{sec:exp-benchmark}, Paragraph 3, Line 1. 


\begin{commentblock}{3-5}
The ‘ComCost’ in Table I is reported but not clearly defined.
\end{commentblock}

\textbf{Response:}
Thank you for your suggestions. 
The 'ComCost' is the inter-chiplet communication costs. 
The communication cost is the multiplication of the data movement frequency with the wirelength between two chiplets.
Longer wirelength will bring more latency in RDLs in chiplet-based architecture.
If frequent data movement occurs between two chiplet with too long distances, the overall performance of the design will deduct heavily.
Because data movement costs can bring more waiting time between components.
Therefore, by using this metric, we can evaluate that our method reduces the communication cost.

\textbf{Action:} 
We add more descriptions from \Cref{sec:exp-result}, Paragraph 3, Line 5. 

\begin{commentblock}{3-6}
The data movement frequency (Section III, part D, paragraph 7) is not clearly defined. Does the communication frequency between chiplets consider data volume?
\end{commentblock}

\textbf{Response:}
Thank you for pointing out the point that is not clearly defined.
In the simulation platform, the communication frequency between chiplets considers the data volume. 
In our \textbf{simChiplet}, the data are sent or received in packages, which have an equal volume. In this way, more data movement frequency can be seen as more data movement volume. 

\textbf{Action:} 
More descriptions are added in \Cref{sec:method-overview}, Paragraph 4, Line 6, where the ``data movement frequency" appears for the first time. 



\begin{commentblock}{3-7}
The non-overlap constraints (Section III, part D, paragraph 3) imply that two chiplets can be exactly adjacent to each other. Is it allowable in a chiplet floorplan?
\end{commentblock}

\textbf{Response:}
Thanks for your reminder.
In practical chiplet-based architecture, there exists a small distance to allow routing wire between two near chiplets.
However, the chiplet floorplan is just a stage of designing a chiplet-based architecture, which is not the final layout solution for manufacturing.
In our framework, the floorplan solutions will be sent to the next stage, \textit{i.e.}, the routing of wires between chiplets in redistribution layers (RDLs).
In the routing stage, the adjacent chiplet will be slightly separated to allow wire routability between them.
Therefore, we think it is a reasonable constraint in floorplan stages.

\textbf{Action:} 
We have added more background information in \Cref{sec:method-optChiplet}, Paragraph 3, Line 3. 



\begin{commentblock}{3-8}
The values of user-defined coefficients in the objective function are not reported in the experiment section.
\end{commentblock}

\textbf{Response:}
We sincerely thank the reviewer for the reminder. 
The order of the magnitude of metrics is different, so the magnitude of user-defined coefficients is different as well.
The user-define coefficients are set based on some pre-experiments to obtain a good tradeoff between multiple objectives and ensure convergence of optimization.
According to pre-experiments, $\beta_{1}$, $\beta_{2}$, $\beta_{3}$, $\beta_4$, and $\gamma_{1}$ in \Cref{equ:final-objective} are set to 1, 10, 100, 1, and 1, respectively. 
The floorplan results demonstrate this setting can achieve a balance between multiple objectives. 

\textbf{Action:} 
We have added all user-defined coefficients in \Cref{sec:exp-result}, Paragraph 2, Line 3.

\section*{\textbf{Associate Editor}}

\begin{commentblock}{}
All three reviewers have raised concerns on the literature review, contributions and experiments. The authors are requested to address all the concerns in a thorough revision.
\end{commentblock}

\textbf{Response:}
The comments and suggestions provided by the reviewers are very valuable, and we have used these insights to improve our manuscript significantly.
We tried our best to improve the manuscript and made some changes marked in blue in the revised paper which will not influence the content and framework of the paper.
We appreciate for Editors/Reviewers’ warm work earnestly, and hope the correction will meet with approval.
Once again, thank you very much for your comments and suggestions.





==> doc/cover.tex <==
{
\twocolumn[
\begin{@twocolumnfalse}
\large

Dear Editor and Reviewers,

\ \\
Thank you very much for reviewing our submission and providing your valuable comments.

\ \\
We have revised this version by addressing reviewers' comments and incorporating their suggestions.

All the recent changes in the current version are highlighted in \revise{blue} color in the updated manuscript.
Detailed responses to reviewers' comments are appended at the end of this manuscript.
The original version of the manuscript is also located at the end for reference.
\ \\
Best regards,

\ \\
Shixin Chen

\end{@twocolumnfalse}
]
}

